Weak measurement of the Goos-Hanchen shift

It is well known from quantum mechanics that weak measurements offer a means of amplifying and detecting very small phenomena. We present here the first experimental observation of the Goos-Hanchen shift via a weak measurement approach.

==> letter.tex <==
@ARTICLE{Goos47,
   author = "F. Goos and H. $\rm H\ddot{\textbf{a}}nchen$",
   year = "1947",
   journal = "Ann.\ Phys.",
   Title = {{Ein neuer und fundamentaler Versuch zur Totalreflexion}},
   volume = "1",
   pages = "333"
}

@ARTICLE{Imbert72,
   author = "C. Imbert",
   year = "1972",
   journal = "Phys. Rev. D",
   Title={{Calculation and Experimental Proof of the Transverse Shift Induced by Total Internal Reflection of a Circularly Polarized Light Beam}},
   volume = "5",
   pages = "787"
}

@ARTICLE{Fedorov55,
   author = "F. I. Fedorov",
   year = "1955",
   journal = "Dokl. Akad. Nauk. Nauk SSSR",
   Title={{K Teorii Polnogo Otrazheniya}},
   volume = "105",
   pages = "465"
}


@ARTICLE{Hesselink06,
   author = "X. Yin and L. Hesselink",
   year = "2006",
   journal = "Appl.\ Phys.\ Lett.",
   Title = {{Goos-H$\rm \ddot{\textbf{a}}$nchen shift surface plasmon resonance sensor}},
   volume = "89",
   pages = "261108"
}


@article{ Merano09,
Author = "Merano, M. and Aiello, A. and van Exter, M. P., and Woerdman, J. P.",
   year = "2009",
   journal = "Nat. Photon.",
   Title={{Observing angular deviations in the specular reflection of a light beam}},
   volume = "3",
   pages = "337"
}

@article{ Kwiat08,
Author = "O. Hosten, and P. Kwiat",
   year = "2008",
   journal = "Science",
  Title={{Observation of the Spin Hall Effect of Light via Weak Measurements}},
   volume = "319",
   pages = "787"
}

@article{ Onoda04,
Author = {Onoda, M and Murakami, S and Nagaosa, N},
Journal = {{Phys. Rev. Lett.}},
Title = {{Hall effect of light}},
Year = {{2004}},
Volume = {{93}},
  pages = "083901"
}

@article{Bliokh06, 
Author = "K. Yu. Bliokh, and Y. P. Bliokh",
   year = "2006",
   Title={{Conservation of Angular Momentum, Transverse Shift, and Spin Hall Effect in Reflection and Refraction of an Electromagnetic Wave   Packet}},
  journal = "Phys. Rev. Lett.",
   volume = "96",
   pages = "073903"
}

@article{ Merano10,
Author = {Merano, M. and Hermosa, N. and Woerdman, J. P. and Aiello, A.},
Title = {{How orbital angular momentum affects beam shifts in optical reflection}},
Journal = {{Phys. Rev. A}},
Year = {{2010}},
Volume = {{82}},
   pages = "023817"
}

@ARTICLE{Bretenaker01,
   author = "C. Bonnet and D. Chauvat and O. Emile and F. Bretenaker and A. Le Floch and L. Dutriaux",
   year = "2001",
   journal = "Opt.\ Lett.",
   volume = "26",
   pages = "666"
}

@article{ Boardman07,
Author = {Tsakmakidis, K. L. and Boardman, A. D. and Hess, O.},
Title = {{`Trapped rainbow' storage of light in metamaterials}},
Journal = {{Nature}},
Year = {{2007}},
Volume = {{450}},
Number = {{7168}},
Pages = {{397}}
}

@article{ Martina06,
Author = {Schomerus, H. and Hentschel, M.},
Title = {{Correcting ray optics at curved dielectric microresonator interfaces:
   Phase-space unification of Fresnel filtering and the Goos-Hanchen shift}},
Journal = {{Phys. Rev. Lett.}},
Year = {{2006}},
Volume = {{96}},
Pages = {{243903}}
}

@article{ Felbacq04,
Author = {Felbacq, D and Sma$\hat{a}$li, R},
Title = {{Bloch modes dressed by evanescent waves and the generalized Goos-Hanchen
   effect in photonic crystals}},
Journal = {{Phys. Rev. Lett.}},
Year = {{2004}},
Volume = {{92}},
Pages = {{193902}}
}

@article{Bliokh12, 
Author = "K. Yu. Bliokh, and F. Nori",
   year = "2012",
   journal = "Phys.\ Rev.\ Lett.",
   volume = "108",
   pages = "120403"
}

@article{ Tamir89,
Author = {Simon, R and Tamir, T},
Title = {{NONSPECULAR PHENOMENA IN PARTLY COHERENT BEAMS REFLECTED BY MULTILAYERED
   STRUCTURES}},
Journal = {{J. Opt. Soc. Am. A}},
Year = {{1989}},
Volume = {{6}},
Number = {{1}},
Pages = {{18}}
}

@article{ Zubairy08,
Author = {Wang, Li-Qin and Wang, Li-Gang and Zhu, Shi-Yao and Zubairy, M. Suhail},
Title = {{The influence of spatial coherence on the Goos-Hanchen shift at total
   internal reflection}},
Journal = {{J. Phys. B}},
Year = {{2008}},
Volume = {{41}},
   pages = "1057"
}

@article{ Aiello08,
Author = {Aiello, A. and Woerdman, J. P.},
Title = {{Role of beam propagation in Goos-Hanchen and Imbert-Fedorov shifts}},
Journal = {{Opt. Lett.}},
Year = {{2008}},
Volume = {{33}},
Pages = {{1437}}
}

@article{ Aiello12,
Author = {Aiello, Andrea and Woerdman, J. P.},
Title = {{Role of spatial coherence in Goos-Hanchen and Imbert-Fedorov shifts:
   reply to comment}},
Journal = {{Opt. Lett.}},
Year = {{2012}},
Volume = {{37}},
Number = {{6}},
Pages = {{1057}}
}

@article{ Aiello11,
Author = {Aiello, Andrea and Woerdman, J. P.},
Title = {{Role of spatial coherence in Goos-Hanchen and Imbert-Fedorov shifts}},
Journal = {{Opt. Lett.}},
Year = {{2011}},
Volume = {{36}},
Number = {{16}},
Pages = {{3151}}
}

@article{ Wang12,
Author = {Wang, Li-Gang and Liu, Ke-Hong},
Title = {{Role of spatial coherence in Goos-Hanchen and Imbert-Fedorov shifts:
   comment}},
Journal = {{Opt. Lett}},
Year = {{2012}},
Volume = {{37}},
Number = {{6}},
Pages = {{1056}}
}

@article{ Gori78,
Author = {Gori, F. and Palma, C.},
Journal = {{Opt. Comm}},
Year = {{1978}},
Volume = {{27}},
Pages = {{185}}
}

@BOOK{Mandel,
  author =       {Mandel, L. and Wolf, E.},
  title =        {Optical Coherence and Quantum Optics},
  publisher =    {Cambridge University Press},
  year =         {1995},
  edition =      {first},
Pages = {{276-287}}
}

@BOOK{Kliger,
  author =       {Kliger, D. S. and Lewis, J. W. and Randall, C. E.},
  title =        {Polarized light in optics and spectroscopy},
  publisher =    {Academic Press},
  year =         {1990},
  edition =      {first},
Pages = {{66}}
}


@article{ Haan10,
Author = {de Haan, Victor-O. and Plomp, Jeroen and Rekveldt, Theo M. and Kraan,
   Wicher H. and van Well, Ad A. and Dalgliesh, Robert M. and Langridge,
   Sean},
Title = {{Observation of the Goos-Hanchen Shift with Neutrons}},
Journal = {{Phys. Rev. Lett.}},
Year = {{2010}},
Volume = {{104}},
Pages = {{010401}}
}

@article{ Martienssen64,
Author = {Martienssen, W. and Spiller, E},
Journal = {{American Journal of Physics}},
Year = {{1964}},
Volume = {{32}},
Pages = {{919}}
}


@article{ Merano12,
Author = {Merano, M. and Umbriaco, G. and Mistura, G.},
Title = {{Observation of nonspecular effects for Gaussian Schell-model light beams}},
Journal = {{Phys. Rev. A}},
Year = {{2012}},
Volume = {{86}},
Pages = {{033842}},
}

@article{Wolfgang12,
Author = {Loffler, W. and Aiello, Andrea and Woerdman, J. P.},
Title = {{Spatial Coherence and Optical Beam Shifts}},
Journal = {{Phys. Rev. Lett.}},
Year = {{2012}},
Volume = {{109}},
Pages = {{213901}},
}

@article{Merano102,
Author = {Merano, M. and Hermosa, N. and Aiello, A. and Woerdman, J. P.},
Title = {{Demonstration of a quasi-scalar angular Goos-Hanchen effect}},
Journal = {{Opt. Lett}},
Year = {{2010}},
Volume = {{35}},
Number = {{21}},
Pages = {{3562-3564}},
Month = {{NOV 1}},
Abstract = {{We show experimentally that the angular Goos-Hanchen (GH) effect can be
   easily observed, also without employing its resonant enhancement at
   Brewster incidence. An s-polarized beam was used to decouple the
   polarization from the propagation dynamics of the beam. We found that,
   in this case, the angular GH effect can be strongly enhanced by
   increasing the angular aperture of the Gaussian beam. Our experiments
   suggest a route toward observing the angular GH effect for true scalar
   waves, such as acoustic waves and quantum matter waves. (C) 2010 Optical
   Society of America}},
Publisher = {{OPTICAL SOC AMER}},
Address = {{2010 MASSACHUSETTS AVE NW, WASHINGTON, DC 20036 USA}},
Type = {{Article}},
Language = {{English}},
Affiliation = {{Merano, M (Reprint Author), Leiden Univ, Huygens Lab, POB 9504, NL-2300 RA Leiden, Netherlands..
   Merano, M.; Hermosa, N.; Woerdman, J. P., Leiden Univ, Huygens Lab, NL-2300 RA Leiden, Netherlands.
   Aiello, A., Max Planck Inst Sci Light, D-91058 Erlangen, Germany.}},
ISSN = {{0146-9592}},
Keywords-Plus = {{DIELECTRIC INTERFACE; LIGHT-BEAMS; REFLECTION; SHIFTS; POLARIZATION}},
Research-Areas = {{Optics}},
Web-of-Science-Categories  = {{Optics}},
Author-Email = {{merano@molphys.leidenuniv.nl}},
ResearcherID-Numbers = {{Aiello, Andrea/A-7518-2012
Hermosa, Nathaniel /G-2237-2012}},
Funding-Acknowledgement = {{European Commission {[}255914]; Alexander von Humboldt Foundation}},
Funding-Text = {{This work is part of the program of the foundation for ``Fundamenteel
   Onderzoek der Materie{''}; it is also supported by the European
   Commission as part of the FET-Open program 255914 ({''}PHORBITECH{''}).
   A. A. acknowledges support from the Alexander von Humboldt Foundation.}},
Number-of-Cited-References = {{24}},
Times-Cited = {{5}},
Journal-ISO = {{Opt. Lett.}},
Doc-Delivery-Number = {{673IW}},
Unique-ID = {{ISI:000283653900009}},
}



@article{Ritchie91,
Author = {Ritchie, NWM and Story, JG and Hulet, RG},
Title = {{REALIZATION OF A MEASUREMENT OF A WEAK VALUE}},
Journal = {{Phys. Rev. Lett.}},
Year = {{1991}},
Volume = {{66}},
Number = {{9}},
Pages = {{1107-1110}},
Month = {{MAR 4}},
Abstract = {{We present the first realization of a measurement of a ``weak value,{''}
   a concept recently introduced by Aharonov, Albert, and Vaidman (AAV). 
   Our experiment uses a birefringent crystal to separate the two
   linear-polarization components of a laser beam by a distance small
   compared to the laser-beam waist.  This ``weak measurement{''} is
   followed by a strong measurement which translates the centroid of the
   beam by a distance far larger than the birefringence-induced separation.
   In addition, we present data corresponding to orthogonal initial and
   final states, for which the weak value is not defined.  This
   interference effect may have application in the amplification and
   detection of weak effects.'}},
Publisher = {{AMERICAN PHYSICAL SOC}},
Address = {{ONE PHYSICS ELLIPSE, COLLEGE PK, MD 20740-3844 USA}},
Type = {{Article}},
Language = {{English}},
Affiliation = {{RITCHIE, NWM (Reprint Author), RICE UNIV,DEPT PHYS,HOUSTON,TX 77251, USA..
   RICE UNIV,RICE QUANTUM INST,HOUSTON,TX 77251.}},
DOI = {{10.1103/PhysRevLett.66.1107}},
ISSN = {{0031-9007}},
Keywords-Plus = {{COMPONENT; SPIN; PARTICLE}},
Research-Areas = {{Physics}},
Web-of-Science-Categories  = {{Physics, Multidisciplinary}},
Number-of-Cited-References = {{9}},
Times-Cited = {{129}},
Journal-ISO = {{Phys. Rev. Lett.}},
Doc-Delivery-Number = {{FA349}},
Unique-ID = {{ISI:A1991FA34900001}},
}


@article{Sudarshan89,
Author = {Duck, IM and Stevenson, PM and Sudarshan, ECG},
Title = {{THE SENSE IN WHICH A WEAK MEASUREMENT OF A SPIN-1/2 PARTICLES SPIN
   COMPONENT YIELDS A VALUE 100}},
Journal = {{Phys. Rev. D}},
Year = {{1989}},
Volume = {{40}},
Number = {{6}},
Pages = {{2112-2117}},
Month = {{SEP 15}},
Publisher = {{AMERICAN PHYSICAL SOC}},
Address = {{ONE PHYSICS ELLIPSE, COLLEGE PK, MD 20740-3844 USA}},
Type = {{Article}},
Language = {{English}},
Affiliation = {{DUCK, IM (Reprint Author), RICE UNIV,DEPT PHYS,TW BONNER NUCL LAB,HOUSTON,TX 77251, USA..
   UNIV TEXAS,DEPT PHYS,CTR PARTICLE THEORY,AUSTIN,TX 78712.
   INST MATH SCI,MADRAS 600113,INDIA.}},
DOI = {{10.1103/PhysRevD.40.2112}},
ISSN = {{0556-2821}},
Research-Areas = {{Astronomy \& Astrophysics; Physics}},
Web-of-Science-Categories  = {{Astronomy \& Astrophysics; Physics, Particles \& Fields}},
Number-of-Cited-References = {{8}},
Times-Cited = {{70}},
Journal-ISO = {{Phys. Rev. D}},
Doc-Delivery-Number = {{AR044}},
Unique-ID = {{ISI:A1989AR04400039}},
}





@article{ Aharonov88,
Author = {Aharonov, Y and Albert, DZ and Vaidman, L},
Title = {{HOW THE RESULT OF A MEASUREMENT OF A COMPONENT OF THE SPIN OF A SPIN-1/2
   PARTICLE CAN TURN OUT TO BE 100}},
Journal = {{Phys. Rev. Lett.}},
Year = {{1988}},
Volume = {{60}},
Number = {{14}},
Pages = {{1351-1354}},
Month = {{APR 4}},
Publisher = {{AMERICAN PHYSICAL SOC}},
Address = {{ONE PHYSICS ELLIPSE, COLLEGE PK, MD 20740-3844 USA}},
Type = {{Article}},
Language = {{English}},
Affiliation = {{AHARONOV, Y (Reprint Author), UNIV S CAROLINA,DEPT PHYS,COLUMBIA,SC 29208, USA..
   TEL AVIV UNIV,SCH PHYS \& ASTRON,IL-69978 TEL AVIV,ISRAEL.}},
DOI = {{10.1103/PhysRevLett.60.1351}},
ISSN = {{0031-9007}},
Research-Areas = {{Physics}},
Web-of-Science-Categories  = {{Physics, Multidisciplinary}},
Number-of-Cited-References = {{2}},
Times-Cited = {{331}},
Journal-ISO = {{Phys. Rev. Lett.}},
Doc-Delivery-Number = {{M7273}},
Unique-ID = {{ISI:A1988M727300002}},
}




@article{ Qin09,
Author = {Qin, Yi and Li, Yan and He, Huanyu and Gong, Qihuang},
Title = {{Measurement of spin Hall effect of reflected light}},
Journal = {{Opt. Lett.}},
Year = {{2009}},
Volume = {{34}},
Number = {{17}},
Pages = {{2551-2553}},
Month = {{SEP 1}},
Abstract = {{We have measured the spin-dependent nanometer-sized displacements of the
   spin Hall effect of the reflected light from a planar air-glass
   interface. In the case of the vertical polarization, the displacement is
   found to increase with the incident angle and subsequently decrease
   after similar to 48 deg, while in the case of the horizontal
   polarization, it changes rapidly near the Brewster angle. For a fixed
   incident angle of 30 deg, the displacement decreases to zero as the
   polarization angle approaches similar to 39 deg from 0 deg (the
   horizontal polarization) and then increases in the opposite direction
   until 90 deg (the vertical polarization). (C) 2009 Optical Society of
   America}},
Publisher = {{OPTICAL SOC AMER}},
Address = {{2010 MASSACHUSETTS AVE NW, WASHINGTON, DC 20036 USA}},
Type = {{Article}},
Language = {{English}},
Affiliation = {{Li, Y (Reprint Author), Peking Univ, State Key Lab Mesoscop Phys, Beijing 100871, Peoples R China..
   Li, Yan, Peking Univ, State Key Lab Mesoscop Phys, Beijing 100871, Peoples R China.
   Peking Univ, Dept Phys, Beijing 100871, Peoples R China.}},
ISSN = {{0146-9592}},
Research-Areas = {{Optics}},
Web-of-Science-Categories  = {{Optics}},
Author-Email = {{li@pku.edu.cn
   qhgong@pku.edu.cn}},
Funding-Acknowledgement = {{National Natural Science Foundation of China (NSFC) {[}10821062];
   National Basic Research Program of China {[}2006CB921601, 2007CB307001]}},
Funding-Text = {{The authors acknowledge financial support from the National Natural
   Science Foundation of China (NSFC) under grant 10821062, and the
   National Basic Research Program of China under grants 2006CB921601 and
   2007CB307001.}},
Number-of-Cited-References = {{12}},
Times-Cited = {{19}},
Journal-ISO = {{Opt. Lett.}},
Doc-Delivery-Number = {{498CO}},
Unique-ID = {{ISI:000270114400003}},
}






@article{Gotte12,
Author = { $\rm G\ddot{o}tte$, J. B. and Dennis, M. R.},
Title = {{Generalized shifts and weak values for polarization components of
   reflected light beams}},
Journal = {{New J. Phys.}},
Year = {{2012}},
Volume = {{14}},
Month = {{JUL 9}},
Abstract = {{The simple reflection of a light beam of finite transverse extent from a
   homogeneous interface gives rise to a surprisingly large number of
   subtle shifts and deflections which can be seen as diffractive
   corrections to the laws of geometrical optics (Goos-Hanchen shifts) and
   manifestations of optical spin-orbit coupling (Imbert-Fedorov shifts),
   related to the spin Hall effect of light. We develop a unified linear
   algebra approach to dielectric reflection which allows for a simple
   calculation of all these effects and lends itself to an interpretation
   of beam shifts as weak values in a classical analogue to a quantum weak
   measurement. We present a systematic study of the shifts for the whole
   beam and its polarization components, finding symmetries between input
   and output polarizations and predicting the existence of material
   independent shifts.}},
Publisher = {{IOP PUBLISHING LTD}},
Address = {{TEMPLE CIRCUS, TEMPLE WAY, BRISTOL BS1 6BE, ENGLAND}},
Type = {{Article}},
Language = {{English}},
Affiliation = {{Gotte, JB (Reprint Author), Max Planck Inst Phys Komplexer Syst, Noethnitzer Str 38, D-01187 Dresden, Germany..
   Goette, J. B., Max Planck Inst Phys Komplexer Syst, D-01187 Dresden, Germany.
   Goette, J. B.; Dennis, M. R., Univ Bristol, HH Wills Phys Lab, Bristol BS8 1TL, Avon, England.}},
DOI = {{10.1088/1367-2630/14/7/073016}},
Article-Number = {{073016}},
ISSN = {{1367-2630}},
Keywords-Plus = {{IMBERT-FEDOROV SHIFTS; GOOS-HANCHEN; SPIN}},
Research-Areas = {{Physics}},
Web-of-Science-Categories  = {{Physics, Multidisciplinary}},
Author-Email = {{joerg.goette@physics.org}},
ResearcherID-Numbers = {{Dennis, Mark/F-9292-2010
Gotte, Jorg/C-4196-2008}},
Funding-Acknowledgement = {{Royal Society}},
Funding-Text = {{We would like to thank Han Woerdman, Konstantin Bliokh, Andrea Aiello,
   Wolfgang Loffler and Martina Hentschel for insightful discussions and
   encouragement. JBG and MRD acknowledge financial support from the Royal
   Society. A considerable part of this work was conducted while JBG was a
   Royal Society Newton Fellow at the University of Bristol.}},
Number-of-Cited-References = {{28}},
Times-Cited = {{3}},
Journal-ISO = {{New J. Phys.}},
Doc-Delivery-Number = {{982UI}},
Unique-ID = {{ISI:000307070500001}},
}




@article{Merano07,
Author = {Merano, M. and Aiello, A. and `t Hooft, G. W. and van Exter, M. P. and
   Eliel, E. R. and Woerdman, J. P.},
Title = {{Observation of Goos-Hanchen shifts in metallic reflection}},
Journal = {{Opt. Exp.}},
Year = {{2007}},
Volume = {{15}},
Number = {{24}},
Pages = {{15928-15934}},
Month = {{NOV 26}},
Abstract = {{We report the first observation of the Goos-Hanchen shift of a light
   beam incident on a bare metal surface. This phenomenon is particularly
   interesting because the Goos-Hanchen shift for p polarized light in
   metals is negative and much bigger than the positive shift for s
   polarized light. The experimental result for the measured shifts as a
   function of the angle of incidence is in excellent agreement with
   theoretical predictions. In an energy-flux interpretation, our
   measurement shows the existence of a backward energy flow at the bare
   metal surface when this is excited by a p polarized beam of light.}},
Publisher = {{OPTICAL SOC AMER}},
Address = {{2010 MASSACHUSETTS AVE NW, WASHINGTON, DC 20036 USA}},
Type = {{Article}},
Language = {{English}},
Affiliation = {{Merano, M (Reprint Author), Leiden Univ, Huygens Lab, POB 9504, NL-2300 RA Leiden, Netherlands..
   Leiden Univ, Huygens Lab, NL-2300 RA Leiden, Netherlands.}},
DOI = {{10.1364/OE.15.015928}},
ISSN = {{1094-4087}},
Keywords-Plus = {{BEAM DISPLACEMENT; ABSORBING MEDIA; INTERFACE}},
Research-Areas = {{Optics}},
Web-of-Science-Categories  = {{Optics}},
Author-Email = {{merano@molphys.leidenuniv.nl}},
Number-of-Cited-References = {{27}},
Times-Cited = {{37}},
Journal-ISO = {{Opt. Express}},
Doc-Delivery-Number = {{235HI}},
Unique-ID = {{ISI:000251223900031}},
}
